Discovery of one neutron star candidate from radial velocity monitoring

We report the discovery of one possible neutron star binary ($P_{\rm orb} =$ 0.8666 day) by using the LAMOST low-resolution spectroscopic data. The visible companion is a late A-type dwarf ($T_{\rm eff} = 7900 \pm 200$ K; log$g$ $=$ 4.3$\pm$0.2; $M =$ 1.7$\pm$0.1 M$_{\odot}$; $R\ =\ 1.7\pm0.2$ R$_{\odot}$), at a distance of 1.11$\pm0.03$ kpc. No double-lined feature can be seen from the GTC/HORuS high-resolution spectra, thus the radial velocity variation indicates an invisible object hiding in the binary. The system's optical light curves show clear ellipsoidal variability, suggesting that the visible companion is tidal distorted. By fitting the multi-band light curves with the ELC and WD codes, we constrain the mass of the invisible star to be 1.1--1.3 M$_{\odot}$. Spectral disentangling shows no additional component with optical absorption spectra, supporting the system contains one compact object. No X-ray or UV emission are detected in the ROSAT archive observations. Therefore, we suspect the invisible object is more likely a neutron star rather than a white dwarf. Our finding suggests the ability of LAMOST spectroscopic survey to discover X-ray quiescent compact objects.

==> rev2_cover_letter.tex <==
Dear Referee,                                                                   
Thanks very much for your comments. 
We have revised our paper (mostly in bold text) taking all your suggestions into account. 
The bold text in last revision is removed. 
Below we present our responses to the issues you brought up. 

Regards,
The authors
----------

I still suggest a few minor points and typos:
. The authors did not explain why the star was observed by LAMOST so many times. Also, are there other stars with so many measurements? Would be nice if the authors can comment on that.

*Response: We add more description in paragraph 1st of Section 2.2.1 (LAMOST observation). This plate is one K2 plate, which was first selected because it includes a lot of photometric variables and RV variables. It also includes LB-1, which was proposed to be a black hole. J06163552 is another interesting target. This plate includes about 3000 stars, meaning about 3000 stars have so many measurements. In addition, there are some other tome-domain plates being surveyed by LAMOST, but the exposure numbers are much less than that of this K2 plate.

. A reference to the optical pulsar: please add the orbital period. Are there any similar systems? 

*Response: Thanks for your comment. Yes there are some similar systems, such as 3FGL J1544.6-1125 (Britt et al. 2017), 3FGL J0954.8-3948 (Li et al. 2018), and a group of pulsars in Strader et al. 2019. However, in the new version, we found the recently published paper about one new discovered quiescent neutron star (Yi et al. 2022) is more approximate being the reference. So we remove the reference of 4FGL J0940.3-7610.

. Detection threshold: in what wavelength range was the test performed?

*Response: The wavelength range used in the test is the same as that in the spectral disentangling, i.e., from 4000 A to 5200 A. We add it in paragraph 3rd of Section 5.1.

. The filling factor appears in the table, but not in the text that discusses it. 

*Response: We add some description in paragraph 1st of Section 5.3. This binary system is only partially Roche lobe filling. This is consistent with the non-detection of X-ray and UV signal, suggesting no accretion disk is present or no accretion exists.



Minor typos:
. Line 131: extra spaceS

* Response: The extra spaces before 'J06163552' seem to be caused by typography, and we have rewrite the sentences.

. 134: space missing

* Response: we have added a space before the reference.

. 434: test -> tests

* Response: we have corrected 'test' to 'tests'.

. 443: reference not properly written

*Response: Done.

====
Dear Allen,

Thank you for sending the referee's report to us. We have revised our paper taking all her/his suggestions into account.

Regards,
The authors

